Bilingual Evaluation of Language Models on General Knowledge in University Entrance Exams with Minimal Contamination

In this article we present UNED-ACCESS 2024, a bilingual dataset that consists of 1003 multiple-choice questions of university entrance level exams in Spanish and English. Questions are originally formulated in Spanish and translated manually into English, and have not ever been publicly released. A selection of current open-source and proprietary models are evaluated in a uniform zero-shot experimental setting both on the UNED-ACCESS 2024 dataset and on an equivalent subset of MMLU questions. Results show that (i) reasoning questions are challenging for models, (ii) smaller models perform worse than larger models and degrade faster in Spanish than in English and (iii) the performance gap between languages is negligible for the best models and grows up to 37% for smaller models. Model ranking on UNED-ACCESS 2024 is almost identical in English and Spanish, and has also a high correlation (0.98 Pearson) with ranking on MMLU, suggesting that a small dataset is sufficiently diverse and representative to measure performance by discipline.

==> apendice_translations.tex <==
\section{Comparison of Multilingual Datasets and Benchmarks}
\label{sec:apendice translations}

Table \ref{traducciones} show a comparison of several multilingual datasets and benchmarks, regarding the languages included, the original language of the questions or instances, whether translations are present or not and the translation method used, and whether the instances in each language are different or the same.

\begin{table*}[ht]
\centering
{\small
\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2.5cm}|p{3.5cm}|}
    \hline
     & \textbf{Languages} & \textbf{Original language of the instances} & \textbf{Translations} & \textbf{Same instances in every language} & \textbf{Translation method} \\ \hline
    \textbf{UNED-ACCESO 2024} & Spanish and English & Spanish & Yes & Yes & Professional manual translations \\ \hline
    \textbf{AGIEval}  \footnotesize{\citep{zhong_agieval_2023}} & English and Chinese & English and Chinese & No translations, except in LogiQA & No, except in LogiQA & Five professional English speakers and three proofreaders to translate manually from Chinese \\ \hline
    \textbf{Xiezhi} \footnotesize{\citep{gu2024xiezhieverupdatingbenchmarkholistic}} & Chinese and English & Chinese & Yes, from Chinese to English & Yes & They use Google Translate API, followed by manual post-processing \\ \hline
    \textbf{M3Exam} \footnotesize{\citep{zhang_m3exam_2023}} & 9 languages & 9 languages & No & No & No translations \\ \hline
    \textbf{EXAMS} \footnotesize{\citep{hardalov-etal-2020-exams}} & 16 languages & 16 languages & No, except for parallel questions & No, except for parallel questions in 7 languages & No translations \\ \hline
    \textbf{XTREME} \footnotesize{\citep{hu2020xtrememassivelymultilingualmultitask}} and \textbf{XTREME-R} \footnotesize{\citep{ruder2021xtremerchallengingnuancedmultilingual}} & 40 languages and 9 tasks (XTREME); 50 languages and 10 tasks (XTREME-R) & Depends on the task$^{*}$ & Depends on the task & Depends on the task & Professional translations, parallel instances and automatic translations$^{**}$
 \\ \hline
    \textbf{MEGA} \footnotesize{\citep{ahuja_mega_2023}} & 70 languages (16 datasets) & Depends on the task & Depends on the task & Depends on the task & Professional translations, parallel instances and automatic translations$^{***}$ \\ \hline
\end{tabular}
}
\caption{Comparison of translation methods in multilingual datasets. ~$^{*}${While in the XNLI \citep{conneau-etal-2018-xnli} or XQuAD \citep{artetxe-etal-2020-cross} datasets the translations from English were done manually by professional translators, in others such as MLQA instances exist naturally in several languages, without relying on English translations.} ~$^{**}${Since not all tasks are available in all languages, to enable a broader comparison across languages they automatically translate some English instances to the remaining languages using an in-house translation system.} ~$^{***}${In order to compare diverse prompting strategies, they use Bing translator to translate target language data to English.}}
\label{traducciones}
\end{table*}









